The Pierre Auger Cosmic Ray Observatory

The Pierre Auger Observatory, located on a vast, high plain in western Argentina, is the world's largest cosmic ray observatory. The objectives of the Observatory are to probe the origin and characteristics of cosmic rays above $10^{17}$ eV and to study the interactions of these, the most energetic particles observed in nature. The Auger design features an array of 1660 water-Cherenkov particle detector stations spread over 3000 km$^2$ overlooked by 24 air fluorescence telescopes. In addition, three high elevation fluorescence telescopes overlook a 23.5 km$^2$, 61-detector infilled array with 750 m spacing. The Observatory has been in successful operation since completion in 2008 and has recorded data from an exposure exceeding 40,000 km$^2$ sr yr. This paper describes the design and performance of the detectors, related subsystems and infrastructure that make up the Auger Observatory.

==> bibliography.tex <==
\begin{thebibliography}{99}
\raggedright

\def\link#1{{\scriptsize\url{#1}}}


\bibitem{auger-39}
  P.~Auger, P.~Ehrenfest, R.~Maze, J.~Daudin, R.A.~Fr\'eon,
  Rev.\ Mod.\ Phys.\ \textbf{11} (1939) 288--291.

\bibitem{Linsley:1963uo}
  J.~Linsley,
  Phys.\ Rev.\ Lett.\ \textbf{10} (1963) 146--148.

\bibitem{nagano00b}
  M.~Nagano \textit{et al.},
  Astropart.\ Phys.\ \textbf{22} (2004) 235--248.

\bibitem{schulz}
  A. Schulz for The Pierre Auger Collaboration,  Proc. 33rd  ICRC (2013), arXiv 1307.5059.

\bibitem{spectrum2008}
  J. Abraham \textit{et al.} [The Pierre Auger Collaboration],
	Phys. Rev. Lett. \textbf{101},  061101 (2008).

\bibitem{largeScale}
  P. Abreu  {\it et al.}  [The Pierre Auger Collaboration], Astropart. Phys. \textbf{34}, 627 (2011). %627Ð639

\bibitem{sidelnik}
  I. Sidelnik for The Pierre Auger Collaboration,  Proc. 33rd  ICRC (2013), arXiv 1307.5059.

\bibitem{rogerio}
  R. M. de Almeida for The Pierre Auger Collaboration,  Proc. 33rd  ICRC (2013), arXiv 1307.5059.

\bibitem{alphaDelta}
  P. Abreu  {\it et al.} [Pierre Auger Collaboration],  Astrophys. J. Lett. \textbf{762}, L13 (2012).

\bibitem{agn}
  J. Abraham {\it et al.}  [The Pierre Auger Collaboration], {\it Astropart. Phys.} \textbf{29}, 188 (2008).

\bibitem{science_2007}
  Pierre Auger Collaboration,
  Science \textbf{318}, 5852 (9 Nov. 2007) 938--943.

\bibitem{xsecPRL}
  P. Abreu  \textit{et al.} [The Pierre Auger Collaboration],  Phys. Rev. Lett. \textbf{109}, 062002 (2012).

\bibitem{lhcXsec}
  T. Cs\"org\"o \textit{et al.}, Prog. Theor. Phys. Suppl. \textbf{193}, 180 (2012).

\bibitem{auger-xmax-2010}
  J.~Abraham \textit{et al.}\ (Pierre Auger Collab.),
  Phys.\ Rev.\ Lett.\ \textbf{104} (2010) 091101.
	
\bibitem{massPRL} J. Abraham \textit{et al.} [The Pierre Auger Collaboration],  Phys. Rev. Lett. \textbf{104}, 091101 (2010)	

\bibitem{lnAJCAP}
  P. Abreu  \textit{et al.} [The Pierre Auger Collaboration], JCAP \textbf{1302}, 026 (2013).

\bibitem{photon}
  M. Settimo for The Pierre Auger Collaboration,
	Proceedings of the International Conference on the Structure and the Interactions of the Photon
	(Photon2013), Paris, 2013.


\bibitem{neutrino} %17
  P. Pieroni for The Pierre Auger Collaboration,  Proc. 33rd  ICRC (2013), arXiv 1307.5059.

\bibitem{design_report}
  \link{http://www.auger.org/technical_info/design_report.html}.

\bibitem{EA_NIM}  %19
  J.~Abraham \textit{et al.}\ (Pierre Auger Collaboration),
  Nucl.\ Instr.\ Methods A \textbf{523} (2004) 50--95.




\bibitem{hybadvantages} %20
  P.~Sommers, Astropart.\ Phys.\ \textbf{3} (1995) 349.

\bibitem{AstPartHybrid}
  B.R.~Dawson, H.Y.~Dai, P.~Sommers, and S.~Yoshida,
  Astropart.\ Phys.\ \textbf{5} (1996) 239.


\bibitem{auger-aperture}
  J.~Abraham \textit{et al.}\ (Pierre Auger Collab.),
  Nucl.\ Instrum.\ Methods A \textbf{613} (2010) 29--39.

\bibitem{HYexpos2011}
  J.~Abraham \textit{et al.}\ (Pierre Auger Collab.),
  Astropart.\ Phys.\ \textbf{34} (2011) 368--381.

\bibitem{auger-espec-2010}
  J.~Abraham \textit{et al.}\ (Pierre Auger Collab.),
  Phys.\ Lett.\ B \textbf{685} (2010) 239--246.

\bibitem{CICHersil}
J.~Hersil \textit{et al.},
  Phys.\ Rev.\ Lett.\ \textbf{6} (1961) 22.


\bibitem{Lodz_angres}
  C.~Bonifazi for the Pierre Auger Collaboration,
  Proc.\ 31st ICRC {\L}\'od\'z, Poland [arXiv:0901.3138] (2009).

\bibitem{ICRC07_dawson}
  B.R.~Dawson for the Pierre Auger Collaboration,
  Proc.\ 30th ICRC (2007) [arXiv:0706.1105].

\bibitem{sd-paper}
  I.~Allekotte \textit{et al.}\ for the Pierre Auger Collaboration,
    Nucl.\ Instrum.\ Methods A \textbf{586} (2008) 408--420.

\bibitem{SD_cal_NIM}
  X.~Bertou \textit{et al.},
  Nucl.\ Instr.\ Methods A \textbf{568} (2006) 839--846.


\bibitem{LUIGI-NIM}
  M.A.L.~de~Oliveira \textit{et al.},
  Nucl.\ Instr.\ Meth.\ A \textbf{522} (2004) 360--370.

\bibitem{Copter-icrc2013}
  J.~Baeuml and M. Unger for the Pierre Auger Collaboration,
  Proc.\ 33th ICRC (2013).

\bibitem{CLFJINST2006}  %32
  B.~Fick, M.~Malek, J.A.J.~Matthew, J.~Matthews, R.~Meyhandan, M.~Mostafa,
  M.~Roberts, P.~Sommers, L.~Wiencke,
  JINST \textbf{1} (2006) P11003.

\bibitem{fdNIM}
  Pierre Auger Collaboration,
  Nucl.\ Instr.\ Methods A \textbf{620} (2010) 227.

\bibitem{calNIM}  %34
  J.T.~Brack \textit{et al.}, JINST 8 (2013) P05014.

\bibitem{LIDARnim2007}  %35
BenZvi S. Y., \textit{et al.},  NIM \textbf{A} 574, (2007) 171.


% offline

\bibitem{Argiro:2007qg}
  S.~Argir\`o, S.L.C.~Barroso, J.~Gonzalez, L.~Nellen, T.~Paul, T.A.~Porter,
  L.~Prado, M.~Roth, R.~Ulrich, and D.~Veberi\v{c},
  Nucl.\ Instrum. Methods Phys. Res. A \textbf{580} (2007) 1485--1496.

\bibitem{xml}
  E.R.~Harold, W.~Scott Means,
  {\em XML in a Nutshell},
  O’Reilly (2004),
  ISBN: 0-596-00764-7;
  \link{http://www.w3.org/XML/}.

\bibitem{python}
  \link{http://www.python.org/}.

\bibitem{root}
  \link{http://root.cern.ch}.

\bibitem{aires}
  S.J.~Sciutto,
  ``AIRES -- A system for air shower simulations'',
  arXiv:astro-ph/9911331.

\bibitem{corsika}
  D.~Heck, J.~Knapp, J.N.~Capdevielle, G.~Schatz, and T.~Thuow,
  Forschungszentrum Karlsruhe Report 6019 (1998).

\bibitem{conex}
  T.~Bergmann, R.~Engel, D.~Heck, N.N.~Kalmykov, S.~Ostapchenko,
  T.~Pierog, T.~Thouw, and K.~Werner,
  Astropart.\ Phys.\ \textbf{26} (2007) 420--432.

\bibitem{seneca}
  H.J.~Drescher, G.~Farrar, M.~Bleicher, M.~Reiter, S.~Soff, and H.~Stoecker,
  Phys.\ Rev.\ D \textbf{67} (2003) 116001.

\bibitem{xerces}
  \link{http://xerces.apache.org/}.

\bibitem{schema}
  \link{http://www.w3.org/standards/xml/schema}.

\bibitem{md5}
  R.~Rivest, RFC 1321: ``The MD5 message-digest algorithm'',
  \link{http://tools.ietf.org/html/rfc1321}.

\bibitem{cppunit}
  \link{http://sourceforge.net/apps/mediawiki/cppunit/}.

\bibitem{buildbot}  %48
  \link{http://buildbot.net/}.

\bibitem{cmake}
  \link{http://www.cmake.org}

\bibitem{ape}
 \link{https://svn.auger.unam.mx/trac/projects/ape/}

\bibitem{cocomo}
  B. Boehm, {\bf Software engineering economics},
  Englewood Cliffs, NJ:Prentice-Hall, 1981. ISBN 0-13-822122-7.

\bibitem{Abreu:2011fb}
  P.~Abreu {\it et al.}  [Pierre Auger Collaboration],
  %``Advanced functionality for radio analysis in the Offline software framework of the Pierre Auger Observatory,''
  Nucl.\ Instrum.\ Meth.\ A {\bf 635}, 92 (2011)
  [arXiv:1101.4473 [astro-ph.IM]].

\bibitem{tunka}
  B.~A.~Antokhonov, D.~Besson, S.~F.~Beregnev, N.~M.~Budnev, O.~B.~Chvalaev, A.~Chiavassa, O.~A.~Gress, N.~N.~Kalmykov {\it et al.},
%  ``A new 1-km**2 EAS Cherenkov array in the Tunka valley,''
  Nucl.\ Instrum.\ Meth.\  {\bf A639}, 42-45 (2011); \\
  {\tt http://heplx3.phsx.ku.edu/~riceuser/ku-tunka/}

\bibitem{Abeysekara:2013tka}
  A.~U.~Abeysekara {\it et al.}  [ HAWC Collaboration],
  %``The HAWC Gamma-Ray Observatory: Design, Calibration, and Operation,''
  arXiv:1310.0074 [astro-ph.IM].
  %%CITATION = ARXIV:1310.0074;%%
  %1 citations counted in INSPIRE as of 20 May 2014

%\cite{Ardouin:2006gj}
\bibitem{Ardouin:2006gj}
  D.~Ardouin, A.~Belletoile, D.~Charrier, R.~Dallier, L.~Denis, P.~Eschstruth, T.~Gousset, F.~Haddad {\it et al.},
%  ``CODALEMA: A cosmic ray air shower radio detection experiment,''
  Int.\ J.\ Mod.\ Phys.\  {\bf A21S1}, 192-196 (2006).


\bibitem{Wyszynski:2012fa}
  O.~Wyszynski, A.~Laszlo, A.~Marcinek, T.~Paul, R.~Sipos, M.~Szuba, M.~Unger and D.~Veberi\v{c},
  %``Legacy code: Lessons from NA61/SHINE offline software upgrade adventure,''
  J.\ Phys.\ Conf.\ Ser.\  {\bf 396}, 052076 (2012).
  %%CITATION = 00462,396,052076;%%

\bibitem{Sipos:2012hs}
  R.~Sipos, A.~Laszlo, A.~Marcinek, T.~Paul, M.~Szuba, M.~Unger, D.~Veberi\v{c} and O.~Wyszynski,
  %``The offline software framework of the NA61/SHINE experiment,''
  J.\ Phys.\ Conf.\ Ser.\  {\bf 396}, 022045 (2012).
  %%CITATION = 00462,396,022045;%%
  %1 citations counted in INSPIRE as of 19 May 2014

%\cite{Ebisuzaki:2014wka}
\bibitem{Ebisuzaki:2014wka}
  T.~Ebisuzaki {\it et al.}  [JEM-EUSO Collaboration],
  %``The JEM-EUSO mission,''
  Adv.\ Space Res.\  {\bf 53}, 1499 (2014).
  %%CITATION = ASRSD,53,1499;%%

\bibitem{FDatmos2010}
  J.~Abraham \textit{et al.}\ (Pierre Auger Collab.),
  Astropart.\ Phys.\ \textbf{33} (2010) 108--129.



\bibitem{GDAS2012}
  P.~Abreu \textit{et al.}\ (Pierre Auger Collab.),
  Astropart.\ Phys.\ \textbf{35} (2012) 591--607.

\bibitem{EPJ2012}
  B.~Keilhauer and M.~Will for the Pierre Auger Collab.,
  Eur.\ Phys.\ J.\ Plus \textbf{127} (2012) 96.

\bibitem{rapidMonit2012}  %52
  P.~Abreu \textit{et al.}\ (Pierre Auger Collab.),
  JINST \textbf{7} (2012) P09001.

\bibitem{Keilhauer2004}
  B.~Keilhauer \textit{et al.},
  Astropart.\ Phys.\ \textbf{22} (2004) 249--261.

\bibitem{Arqueros2008}
  F.~Arqueros, J.~H\"orandel, B.~Keilhauer,
  Nucl.\ Instrum.\ Methods A \textbf{597} (2008) 1--22.

\bibitem{Keilhauer2008}
  B.~Keilhauer \textit{et al.},
  Nucl.\ Instrum.\ Methods A \textbf{597} (2008) 99--104.

\bibitem{Monasor2011}
  M.~Monasor \textit{et al.},
  Astropart.\ Phys.\ \textbf{34} (2011) 467--475.

\bibitem{Keilhauer2012}   %57
  B.~Keilhauer \textit{et al.},
  EPJ web Conf.\ 53 (2013) 01010.
%  Proc. International Symposium on Future Directions in UHECR Physics
%  (CERN, 2012); arXiv:1210.1319.

\bibitem{SDatmos2009}
  J.~Abraham \textit{et al.}\ (Pierre Auger Collab.),
  Astropart.\ Phys.\ \textbf{32} (2009) 89--99.

\bibitem{KeilhauerUnger2009}  %59
  B.~Keilhauer and M.~Unger,
  Proc.\ 31st ICRC, {\L}\'od\'z, Poland, (2009);
  arXiv:0906.5487.


\bibitem{CLFJINST2013}
  P.~Abreu \textit{et al.}\ (Pierre Auger Collab.),
   JINST \textbf{8} (2013) P04009.

\bibitem{LIDAREPJ2012}  %61
V. Rizi, A. Tonachini, \textit{et al.}\ (Pierre Auger Collab.),
EPJ Plus, 127 8 (2012) 92.


\bibitem{Henyey-Greenstein}  %62
  L.G. Henyey, J.L. Greenstein,
	Astrophysical Journal \textbf{93} (1941) 70--83.

\bibitem{fram_GRB}   %63
  M.~Jelinek \textit{et al.},
  Astron.\ Astrophys.\ \textbf{454} (2006) L119.

\bibitem{fram_icrc2007}
  S.~BenZvi \textit{et al.}\ for the Pierre Auger Collaboration,
  Proc.\ 30th ICRC (2007) [arXiv:0706.1710].

\bibitem{WinnickCooperCloud}
  M.G.~Winnick,
    Ph.D.\ thesis, University of Adelaide (2010);
  M.\ Cooper,
  Ph.D.\ thesis, University of Adelaide (2013).





\bibitem{cloudsatellite2012}
 P.~Abreu \textit{et al.}\ (Pierre Auger Collab.),
 Astropart. Phys. 50--52 (2013) 92--101.



\bibitem{icrc2013-cloud}  %67
  J.~Chirinos for the Pierre Auger Collaboration,
  Proc.\ 33th ICRC (2013); arXiv:1307:5059.

\bibitem{EPJ_Summary}
``Focus Point on Interdisciplinary Science with Cosmic Rays," Guest editors: A Bueno, L. Wiencke,
EPJ Plus, \textbf{127} 8 (2012).

\bibitem{EPJ_Elves}
R. Mussa for the Pierre Auger Collaboration,
EPJ Plus, \textbf{127} 94 (2012).



\bibitem{aerosols_Micheletti2012}
  M.~Micheletti et al.,
  Nucl.\ Instrum.\ Methods B \textbf{288} (2012) 10--17.

\bibitem{icrc2013-aerosols}
 M.I.~Micheletti for the Pierre Auger Collaboration et al.,
 Proc.\ 33th ICRC (2013); arXiv:1307:5059.

%\bibitem{VAOD_INST}
%P.~Abreu \textit{et al.}\ (Pierre Auger Collab.),
 %JINST \textbf{8} (2013) P04009.








\bibitem{Ave:2008zza}
M.~{Ave et al. [AIRFLY Collaboration]}, Nucl.\ Instrum.\ Meth. A597 (2008) 41.

\bibitem{Ave:2012ifa}
M.~{Ave et al. [AIRFLY Collaboration]}, Astropart.\ Phys. 42 (2013) 90.

\bibitem{cher:giller}
  M.~Giller, \textit{et al.},
  J.\ Phys.\ G \textbf{30} (2004) 97.

\bibitem{cher:nerling}
  F.~Nerling \textit{et al.},
  Astropart.\ Phys.\ \textbf{24} (2006) 421.

\bibitem{Roberts:2005xv}
  M.D.~Roberts,
  J.\ Phys.\ G \textbf{31} (2005) 1291.

\bibitem{profileReco}
  M.~Unger \textit{et al.},
  Nucl.\ Instrum.\ Meth.\ A \textbf{588} (2008) 433.

\bibitem{lateralFluorescence}
  D.~Gora \textit{et al.},
  Astropart.\ Phys.\ \textbf{24} (2006) 484.

\bibitem{lateralCherenkov}
  B.R.~Dawson, M.~Giller, and G.~Wieczorek,
  Proc.\ 30th ICRC (2007).

\bibitem{ghfunc}
  T.K.~Gaisser and A.M.~Hillas,
  Proc.\ 15th ICRC, \textbf{8} (1977) 353.

\bibitem{icrc13InvE}  %81
M.~{Tueros for the Pierre Auger Collaboration}, {Proc.\ 33nd ICRC (2013),
  arXiv:1307.5059}.

\bibitem{NKG}
  K.~Kamata and J.~Nishimura,
  Prog.\ Theor.\ Phys.\ Suppl.\ \textbf{6} (1958) 93;
  K.~Greisen,
  Prog.\ Cosmic Ray Physics, \textbf{3} (1956) 1.


% radio bibliography
\bibitem{Allan1971}
  H.R.~Allan,
  Progr.\ Part.\ Nucl.\ Phys.\ Cosmic Ray Phys.\ \textbf{10} (1971) 169.

\bibitem{Fegan2012}
  D.J.~Fegan,
  Nucl.\ Instr. Methods A \textbf{662} (2012) S12.

\bibitem{LOPES2005}
  H.~Falcke \textit{et al.},
  Nature \textbf{435} (2005) 313.

\bibitem{CODALEMA2006}
  D.~Ardouin \textit{et al.},
  Astrop.\ Phys.\ \textbf{26} (2006) 341.

\bibitem{RadioOffline}
  The Pierre Auger Collaboration,
  Nucl.\ Instr.\ Methods A \textbf{635} (2011) 92.

\bibitem{RevenuICRC2011}
  B.~Revenu for the Pierre Auger Collaboration,
  Proc.\ 32nd ICRC (2011) \textbf{3} 172;
  arXiv:1107.4807.

\bibitem{KelleyICRC2011}
  J.L.~Kelley for the Pierre Auger Collaboration,
  Proc.\ 32nd ICRC (2011) \textbf{3} 112;
  arXiv:1107.4807.

\bibitem{Fliescher2012}
  The Pierre Auger Collaboration,
  JINST \textbf{7} (2012) P10011.

% microwave bibliography

\bibitem{Gorham2008}
  P.W.~Gorham \textit{et al.},
  Phys.\ Rev.\ D \textbf{78} (2008) 032007.

\bibitem{AllisonICRC2011}
  P.~Allison for the Pierre Auger Collaboration,
  Proc.\ 32nd ICRC (2011) \textbf{3} 137--140;
  arXiv:1107.4807.

\bibitem{Facal2012}
  P.~Facal San Luis for the Pierre Auger Collaboration,
  Proceedings, International Symposium on Future Directions in UHECR Physics (UHECR2012) : CERN, Geneva, Switzerland, February 13-16, 2012;
  EPJ Web Conf.\  {\bf 53}, 08009 (2013).


\bibitem{Alvarez_NIM}
  J.~Alvarez-Mu\~niz \textit{et al.},
  submitted to Nucl.\ Inst.\ Meth.;
  arXiv:1208.2734.

\bibitem{Alvarez2012}
  J.~Alvarez-Mu\~niz \textit{et al.},
  Phys.\ Rev.\ D \textbf{86} (2012) 051104R.

% sd reco


\bibitem{Pesce:ICRC11}
  R.~Pesce for the Pierre Auger Collaboration,
  Proc.\ 32nd ICRC Beijing, China, \textbf{2} (2011) 214--217;
  arXiv:1107.4809.

\bibitem{Dembinski:ICRC11}
  H.P.~Dembinski for the Pierre Auger Collaboration,
  Proc.\ 32nd ICRC Beijing, China, \textbf{2} (2011) 101--104;
  arXiv:1107.4809.

\bibitem{Roth:ICRC07}
  M.~Roth for the Pierre Auger Collaboration,
  Proc.\ 30th ICRC M\'erida, Mexico, \textbf{4} (2007) 327--330.

\bibitem{Ave:ICRC07}
  M.~Ave for the Pierre Auger Collaboration,
  Proc.\ 30th ICRC M\'erida, Mexico, \textbf{4} (2007) 307--310;
  arXiv:0709.2125.

\bibitem{Bertou:ICRC05}
  X.~Bertou for the Pierre Auger Collaboration,
  Proc.\ 29th ICRC Pune, India, \textbf{7} (2005) 1--4.

\bibitem{Ghia:ICRC05}
  P.L.~Ghia for the Pierre Auger Collaboration,
  Proc.\ 29th ICRC Pune, India, \textbf{7} (2005) 167--170.

\bibitem{Bonifazi:ICRC05}
  C.~Bonifazi for the Pierre Auger Collaboration,
  Proc.\ 29th ICRC Pune, India, \textbf{7} (2005) 17--20.

\bibitem{Barnhill:ICRC05}
  D.~Barnhill \textit{et al.}\ for the Pierre Auger Collaboration,
  Proc.\ 29th ICRC Pune, India, \textbf{7} (2005) 291--294.

\bibitem{angular_resolution}
  C.~Bonifazi for the Pierre Auger Collaboration,
  Nucl.\ Phys.\ B Proc.\ Suppl.\ \textbf{190} (2009) 20--25.




% amiga

\bibitem{SanchezICRC2011}
  F.~S\'anchez for the Pierre Auger Collaboration,
  Proc.\ 32th ICRC, Beijing, China, \textbf{3} (2011) 149--152;
  \link{http://www.ihep.ac.cn/english/conference/icrc2011/paper/proc/v3/v3_0742.pdf}.

\bibitem{proc:icrc2011AMIGA_BWundheiler}
  B.~Wundheiler for the Pierre Auger Collaboration,
  Proc.\ 32th ICRC, Beijing, China, \textbf{3} (2011) 84--87;
  \link{http://www.ihep.ac.cn/english/conference/icrc2011/paper/proc/v3/v3_0341.pdf}.

\bibitem{Maris:ICRC11}
  I.~Mari\c{s} for the Pierre Auger Collaboration,
  Proc.\ 32th ICRC, Beijing, China, \textbf{1} (2011) 267--270;
  \link{http://www.ihep.ac.cn/english/conference/icrc2011/paper/proc/v1/v1_0711.pdf};
  arXiv:1107.4809.

\bibitem{paperAMIGA:2011_MPlatino}
  M.~Platino \textit{et al.},
  JINST \textbf{6} (2011) P06006.

\bibitem{AKENO}
  M.~Nagano \textit{et al.},
  J.\ Phys.\ G \textbf{18} (1992) 423--442.

\bibitem{Supanitsky2008}
  A.D.~Supanitsky \textit{et al.},
  Astropart.\ Phys.\ \textbf{29} (2008) 461--470.


\bibitem{vispa}
  \link{http://www.vispa.physik.rwthaachen.de/}.

% other

\bibitem{solar1}
  Advances in Space Research 49 (2012) 1563-1569,
DOI:10.1016/j.asr.2011.12.028 , arXiv:1204.6196.

\bibitem{solar2}
The Pierre Auger Collaboration,
JINST 6, P01003 (2011),
doi:10.1088/1748-0221/6/01/P01003 .

\bibitem{publicEventDisplay}
\link{http://auger.colostate.edu/ED/}.

\bibitem{Inan:1991}
U.~S.~Inan, T.~ F.~ Bell, J.~V.~Rodriguez, Geophys.~Res.~Lett.
\textbf{18}, (1991) 705

\bibitem{Boeck:1992}
W.~L.~Boeck {\it et al.}, Geophys.~Res.~Lett. \textbf{19}, (1992) 99

\bibitem{Fukunishi:1996}
H.~Fukunishi {\it et al.}, Geophys.~Res.~Lett. \textbf{23}, (1996) 2157

\bibitem{Inan:1997}
U.~S.~Inan {\it et al.}, Geophys.~Res.~Lett. \textbf{24}, (1997) 583

\bibitem{Newsome:2010}
R.~T.~Newsome  and U.~T.~Inan, J.Geophys.Res. \textbf{115}, (2010) A00E41

\bibitem{Chen:2008}
A.~B.~Chen, J.Geophys.Res. \textbf{113}, (2008) A08306

\bibitem{Tonachini:2013}
A.Tonachini  {\it et al.}, Proc.ICRC 2013, ArXiV:1307.5059 (2013),112

\bibitem{Greisen}
  K.~Greisen,
  Phys.\ Rev.\ Lett.\ \textbf{16} (1966) 748.

\bibitem{ZK}
  G.T.~Zatsepin, V.A.~Kuzmin,
  Sov.\ Phys.\ JETP Lett.\ \textbf{4} (1966) 78.




\bibitem{FERMILAB-PUB-07-068-E-TD}
  P.~Mantsch for the Auger Collaboration,
  ``The Pierre Auger Project: A Model for International Science,''
  FERMILAB-PUB-07-068-E-TD (2007).







\bibitem{EPJ_sum_2012}
  L.~Wiencke for the Pierre Auger Collab.,
  Eur.\ Phys.\ J.\ Plus \textbf{127} (2012) 98.

\bibitem{HEAT-ICRC2011-Mathes}
  T.H.-J.~Mathes for the Pierre Auger Collaboration,
  Proc.\ 32nd ICRC, Beijing, China, \textbf{3} (2011) 153--156.




\end{thebibliography}


==> glossary.tex <==
% glossary of acronyms and abbreviations

\begin{table*}[th]
\caption{Glossary of acronyms and abbreviations related to the Pierre Auger Observatory.
Abbreviations in common use, e.g., GPS, are not included.}
\label{tab:glossary}
%\begin{center}
\begin{tabular}{ll}
\toprule
AERA			& Auger Engineering Radio Array  \\
AMIGA			& Auger Muon and Infill Ground Array \\
APF				& Aerosol phase function   \\
ARQ				& Automatic repeat request \\
BLS				& Balloon Launching Station  \\
CDAS 			& Central Data Acquisition System  \\
CIC				& Constant Intensity Cut method  \\
CLF				& Central Laser Facility  \\
EAS				& Extensive air shower \\
ELVES			& (defined in Section~\ref{sec:Elves}) \\
FADC			& Flash Analog-to-Digital Convertor \\
FD				& Fluorescence Detector 					\\
FRAM			& Photometric Robotic Atmospheric Monitor \\
GDAS			& Global Data Assimilation System  \\
HAM 			& Horizontal Attenuation Monitor  \\
HEAT			& High-Elevation Auger Telescopes \\
LDF				& Lateral distribution function \\
MD				& Muon Detector \\
PLD				& Programmable logic device  \\
PMT				& Photomultiplier tube  \\
SCS 			& Slow Control System \\
SD				& Surface Detector  \\
SDP				& Shower-detector plane  \\
TDMA			& Time Division Multiple Access \\
ToT       & Time over threshold  \\
VEM				& Vertical Equivalent Muon \\
XLF				& eXtreme Laser Facility \\
\bottomrule
\end{tabular}
%\end{center}
\end{table*}

==> organization.tex <==
\section{Organization and Operation}

\subsection{Organization}
       
The collaboration that emerged during and after the design workshop
now consists of 92 institutions in 18 countries spread over four
continents. No country dominates, and the maximum contribution of any
one country to construction was less than 25\% of the total.  The Auger
project has become a successful model for a broad international
partnership for building science infrastructure
\cite{FERMILAB-PUB-07-068-E-TD}.

The first step in organizing the collaboration was to establish two
oversight bodies - Collaboration Board and Finance Board.  The
Collaboration Board, consisting of representatives from all of the
Auger member institutions, is the oversight body of the collaboration
that deals with such issues as science policy, admission of new
members and publications.  The Finance Board, on the CERN model,
provides financial oversight and consists of designees from each of the funding agencies.

The next organizational step was to develop an international
agreement.  A draft agreement was developed that was a synthesis of
governance schemes from collider experiments and large astronomy
projects.  The Auger International Agreement is a simple, non-binding
statement of support for the project together with concise statements
on financing, membership, withdrawal, ownership and related governance
issues.

Below the Finance Board and Collaboration Board in the Auger
organization are the spokespersons and the project office.  The
project management office staff consists of the project manager,
deputy project manager, the project engineer and personnel for cost
and schedule quality assurance and safety.  Task Leaders coordinate
the work of Task Groups for each of the detector subsystems, data acquisition, 
data processing, communications and data analysis.

\subsection{Operation}

The Site Management Organization for the Pierre Auger Observatory in Argentina has 
a staff of 32 physicists, engineers and technicians and is headed by the Site Manager.  
The Observatory staff is responsible for the routine maintenance of the detector systems and 
infrastructure under the direction of the project Task Groups.  The support by every Auger 
institution for the operation of the Observatory, including serving shifts, 
non-routine equipment repair, data processing and upgrades is defined in a 
Memorandum of Understanding for Operations.  An independent foundation, 
Fundaci\'{o}n Observatorio Pierre Auger Argentina (FOPAA) was formed to act as 
legal agent for the Auger Project in Argentina.  FOPAA enables hiring of staff, 
holding contracts and handling operating funds for the Observatory within Argentina.  
Operations cost sharing among Auger countries is based on a list of all 
collaborators (excluding students) eligible to sign scientific papers.

